Towards Stability Analysis of Data Transport Mechanisms: a Fluid Model and an Application

The Transmission Control Protocol (TCP) utilizes congestion avoidance and control mechanisms as a preventive measure against congestive collapse and as an adaptive measure in the presence of changing network conditions. The set of available congestion control algorithms is diverse, and while many have been studied from empirical and simulation perspectives, there is a notable lack of analytical work for some variants. To gain more insight into the dynamics of these algorithms, we: (1) propose a general modeling scheme consisting of a set of functional differential equations of retarded type (RFDEs) and of the congestion window as a function of time; (2) apply this scheme to TCP Reno and demonstrate its equivalence to a previous, well known model for TCP Reno; (3) show an application of the new framework to the widely-deployed congestion control algorithm TCP CUBIC, for which analytical models are few and limited; and (4) validate the model using simulations. Our modeling framework yields a fluid model for TCP CUBIC. From a theoretical analysis of this model, we discover that TCP CUBIC is locally uniformly asymptotically stable -- a property of the algorithm previously unknown.

==> Agreement.tex <==
%\subsection{Agreement Between the ODEs and Linearized Model}
\begin{figure*}[th!]
\centering
\subfloat[time={[0,5]}s]{
\includegraphics[width=0.45\textwidth]{figsReno/ODEsVSLinear.pdf}
}
\subfloat[time={[0,1]}s]{
\includegraphics[width=0.45\textwidth]{figsReno/ODEsVSLinearZoomed.pdf}
}
\caption{ODEs vs linearized model. $C=1$, $\tau=0.1$.}
\label{fig:odevslin}
\end{figure*}
We pick values of $C$ and $\tau$ to ensure stability of both the ODEs and the linearized models. Figure \ref{fig:odevslin} shows the comparison between the two systems. The steady-state values of all four systems are the same. The transient behaviors of models A and B seem identical (the blue and magenta curves match exactly), as do the transient behaviors of the linearized versions of models A and B (the cyan and green curves match exactly). The transient behaviors of the original systems and linearized systems have a very close match.

==> Convergence_2.tex <==
%\subsubsection*{Boundedness}
Next, we derive a function $w$.
Recall that we have shown that
\begin{align*}
%\dot{V} &= d_1\left(-\alpha x_1^4+\beta x_1^3x_2-\gamma x_1^2x_2^2\right)-\frac{d_4}{\hat{s}}x_2^4 +h.o.t.
\dot{V} &= \vect{y}^TQ\vect{y} +h.o.t.
\end{align*}
where $Q$ is negative definite and the higher-order terms have combined powers of at least 4.5 in $x_1$ and $x_2$.
%We can express the lower-order terms in matrix form, as follows:
By using a different symmetrization of the lower-order terms $\vect{y}^TQ\vect{y}$, we can obtain the following:
\begin{align*}
\dot{V} &= -\vect{z}^T\tilde{Q}\vect{z}+h.o.t.
\end{align*}
\begin{align*}
\text{where } \vect{z}=\begin{bmatrix}
x_1^2 \\[0.3em]
\sqrt{2}x_1x_2 \\[0.3em]
x_2^2
\end{bmatrix} \text{ and }
\tilde{Q}=
\begin{bmatrix}
d_1\alpha & -\frac{d_1\beta}{2\sqrt{2}} & 0\\[0.3em]
-\frac{d_1\beta}{2\sqrt{2}} & \frac{d_1\gamma}{2} & 0\\[0.3em]
0 & 0 & d_4/\shat
\end{bmatrix}
\end{align*}
%Let's call the matrix above $\tilde{Q}$. 
Since we have previously shown that the sum of the lower-order terms in $\dot{V}$ is a negative definite function, it follows that $\tilde{Q}$ is positive definite, so all of its eigenvalues are strictly positive. Since $\tilde{Q}$ is a real and symmetric matrix, its Rayleigh quotient is bounded below by its smallest eigenvalue $\lambda_{\min}[\tilde{Q}]$. Hence, 
\begin{align*}
\dot{V} &\leq -\lambda_{\min}[\tilde{Q}] \left|\left|\begin{bmatrix}
x_1^2 \\[0.3em]
\sqrt{2}x_1x_2 \\[0.3em]
x_2^2
\end{bmatrix}\right|\right|_2^2+h.o.t.\\
%&=  -\lambda_{\min}[\tilde{Q}] (x_1^4+2x_1^2x_2^2+x_2^4)+h.o.t.\\
&= -\lambda_{\min}[\tilde{Q}] ||\vect{x}||_2^4+h.o.t.
\end{align*}
%Previously, we showed that the higher-order terms have orders of at least $4.5$. 
%Then 
For $|x_1|,$ $|x_2|$ small enough, there exists a positive constant $K$ such that
\begin{align*}
h.o.t. \leq K||\vect{x}||_2^4
\end{align*}
\begin{claim}
\label{claim:limK}
\begin{align*}
&\text{Let }f(x_1,x_2) =\frac{h.o.t.}{||\vect{x}||_2^4}.\\
&\text{We claim that } \lim\limits_{(x_1,x_2)\to (0,0)}\frac{h.o.t.}{||\vect{x}||_2^4}=0.
\end{align*}
\noindent\textbf{Proof:} To prove our claim, we will show that for every $\epsilon>0$, there exists a $\delta >0$ so that whenever $0<\sqrt{x_1^2+x_2^2}<\delta$, $|f(x_1,x_2)|<\epsilon$.
The higher-order terms are a sum of terms that have format $c_0x_1^{c_1}x_2^{c_2}$, where $c_0$ is either a constant or a function of $x_{1_{\theta+\tau}}$ and $x_{2_{\theta+\tau}}$, as in the case of the higher-order terms that arise from the $x_2^3\dot{x}_{1_{\theta}}\tau$ term of $\dot{V}$. In addition, $c_1+c_2\geq 4.5$.
Let $n$ be the number of higher-order terms. Then we can write $|f(x_1,x_2)|$ as follows:
\begin{align*}
|f(x_1,x_2)| &=\frac{1}{||\vect{x}||_2^4}\left|\sum\limits_{i=1}^n c_0^{(i)}x_1^{c_1^{(i)}}x_2^{c_2^{(i)}}\right|
\end{align*}
where the superscript $(i)$ corresponds to the $i$th higher-order term.
\begin{align*}
|f(x_1,x_2)| &\leq \frac{1}{||\vect{x}||_2^4}\sum\limits_{i=1}^n \left|c_0^{(i)}x_1^{c_1^{(i)}}x_2^{c_2^{(i)}}\right|
\end{align*}
Consider any term $|c_0x_1^{c_1}x_2^{c_2}|$. Factor out any combination $|x_1|^a|x_2|^b$ such that $a+b=4$. We know that 
\begin{align*}
|x_1|,|x_2|\leq \sqrt{x_1^2+x_2^2}
\end{align*}
Then 
\begin{align*}
|x_1|^a|x_2|^b &\leq \left(\sqrt{x_1^2+x_2^2}\right)^4 = ||\vect{x}||_2^4\\
|c_0x_1^{c_1}x_2^{c_2}| &\leq |c_0g(x_1,x_2)|||\vect{x}||_2^4
\end{align*}
where $g(x_1,x_2)$ is defined s.t. $g(x_1,x_2)x_1^ax_2^b=x_1^{c_1}x_2^{c_2}$.
\begin{align*}
|f(x_1,x_2)| &\leq \frac{1}{||\vect{x}||_2^4}\sum\limits_{i=1}^n \left|c_0^{(i)}g^{(i)}(x_1,x_2)\right|||\vect{x}||_2^4\\
|f(x_1,x_2)| &\leq  \sum\limits_{i=1}^n \left|c_0^{(i)}g^{(i)}(x_1,x_2)\right|
\end{align*}
Each function $g(x_1,x_2)$ necessarily has the form
\begin{align*}
g(x_1,x_2) &= x_1^{l_1}x_2^{l_2},\ l_1,l_2\geq 0,\ l_1+l_2\geq \frac{1}{2}
\end{align*}
Hence, we can bound the absolute value of each of these functions by a function of $\delta$.
\begin{align*}
|x_{1/2}| &\leq \sqrt{x_1^2+x_2^2}<\delta\\
|x_{1/2}|^{l_{1/2}} &\leq \left(\sqrt{x_1^2+x_2^2}\right)^{l_{1/2}} <\delta^{l_{1/2}}\\
|g(x_1,x_2)| &\leq \left(\sqrt{x_1^2+x_2^2}\right)^{l_1+l_2} < \delta^{l_1+l_2}
\end{align*}
This gives us
\begin{align*}
|f(x_1,x_2)| &\leq \sum\limits_{i=1}^n \left|c_0^{(i)}\right|\delta^{l_1^{(i)}+l_2^{(i)}}
\end{align*}
We would like the sum above to be less than a given $\epsilon>0$. We can always find a $\delta>0$ small enough to make this happen. \qed
\end{claim}
By Claim \ref{claim:limK}, we can always find a $K$ small enough by restricting $x_1$ and $x_2$ into a smaller neighborhood around $\vect{0}$. Hence, we can find a $K<\lambda_{\min}[\tilde{Q}]$, which would give us:
\begin{align}
\label{bound:vdot}
\dot{V} &\leq -(\lambda_{\min}[\tilde{Q}]-K) ||\vect{x}||_2^4
\end{align}
where $\lambda_{\min}[\tilde{Q}]-K>0$. By inspection, we have found a $w(||\vect{x}||)$ that satisfies condition (\ref{eq:Vdotw}) under (\ref{eq:Vdotcondstr}). In addition, 
$w(||\vect{x}||))>0$ when $||\vect{x}||>0$, as necessary. Finally, $\lim_{||\vect{x}||\to\infty}u(||\vect{x}||)=\infty$. We have shown that the function that drives CUBIC's \cwnd, (\ref{eq:cubiccwnd}), is locally uniformly asymptotically stable.
%We will now bound the higher-order terms. Recall that these terms have three components: the first comes from the $x_2^3\dot{x}_{1_{\theta}}\tau$ term, the second from $d_1x_1R_{\vect{0},6}^1$, and the third from $d_4x_2^3R_{\vect{0},3}$
\subsection{Convergence}
Using the Lyapunov-Razumikhin function and its derivative, it is possible to explicitly demonstrate the convergence of trajectories to the fixed point.
Recall that 
\begin{align*}
V(\vect{x}) &\leq \epsilon_0||\vect{x}||_2^2
\ \rightarrow\ V^2(\vect{x}) \leq \epsilon_0^2||\vect{x}||_2^4
\end{align*}
Combined with (\ref{bound:vdot}), this gives us
\begin{align*}
\dot{V} &\leq -\frac{(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}V^2%\\
%\frac{\dot{V}}{V^2} &\leq -\frac{(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}
\end{align*}
We can solve this differential inequality and obtain
\if{false}
We now solve this differential inequality.
We note that 
\begin{align*}
\frac{d}{dt}\left(-\frac{1}{V}\right)&=\frac{\dot{V}}{V^2}\leq -\frac{(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}\\
\frac{d}{dt}\left(\frac{1}{V}\right)&\geq\frac{(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}
\end{align*}
Applying a definite integral on both sides,
\begin{align}
%\int_0^t \frac{d}{ds}\left(\frac{1}{V}\right)ds = \frac{1}{V(t)}-\frac{1}{V(0)} &\geq \int_0^t\frac{(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}ds=\frac{(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}t\\
\int_{t_0}^t \frac{d}{ds}\left(\frac{1}{V}\right)ds &\geq \int_{t_0}^t\frac{(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}ds%=\frac{(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}t\\
\label{eq:integ}
\end{align}
By the fundamental theorem of calculus,
\begin{align}
\int_{t_0}^t \frac{d}{ds}\left(\frac{1}{V}\right)ds = \frac{1}{V(t)}-\frac{1}{V(t_0)}
\label{eq:fundthm}
\end{align}
Evaluating the right-hand side of (\ref{eq:integ}) and combining with (\ref{eq:fundthm}),
\begin{align*}
\frac{1}{V(t)}-\frac{1}{V(t_0)} &\geq \frac{(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}(t-t_0)\\
\frac{1}{V(t)} &\geq \frac{(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}(t-t_0)+\frac{1}{V(t_0)}\\
V(t) &\leq \frac{1}{\frac{(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}(t-t_0)+\frac{1}{V(t_0)}}
\end{align*}
\fi
\begin{align*}
V(t) &\leq \frac{1}{\frac{(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}(t-t_0)+\frac{1}{V(t_0)}}
\end{align*}
Since $V(t)\geq \epsilon_1||\vect{x}||_2^4$,
\begin{align}
||\vect{x}||_2^4 \leq \frac{1}{\frac{\epsilon_1(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}(t-t_0)+\frac{\epsilon_1}{V(t_0)}}
\label{eq:xbound}
\end{align}
We can simplify this bound using the definition of uniform stability:
\begin{definition}[Definition 1.1 from \cite{gu2003stability}]
For the system described by (\ref{eq:rfde}), the trivial solution $x(t)=0$ is said to be stable if for any $t_0\in\mathbb{R}$ and any $\epsilon>0$, there exists a $\delta(t_0,\epsilon)>0$ such that $||x_{t_0}||_c<\delta$ implies $||x(t)||<\epsilon$ for $t>t_0$. It is said to be uniformly stable if it is stable and $\delta(t_0,\epsilon)$ can be chosen independently of $t_0$. It is uniformly asymptotically stable if it is uniformly stable and there exists a $\delta_a>0$ such that for any $\eta>0$, there exists a $T(\delta_a,\eta)$, such that $||x_{t_0}||_c<\delta_a$ implies $||x(t)||<\eta$ for $t\geq t_0+T$ and $t_0\in\mathbb{R}$.
\end{definition}
Above, $||\phi||_c=\max_{a\leq\xi\leq b}||\phi(\xi)||$ for $\phi\in\mathcal{C}[a,b]$ and $x_{t_0}=\phi$ or $x(t_0+\theta)=\phi(\theta)$, $-\tau\leq\theta\leq 0$. 
%For our system, given an $\epsilon>0$, $\exists$ a $\delta(\epsilon)>0$ s.t. $||\vect{x}(t)||<\epsilon$, $\forall\ t$ when $||\vect{x}(t_0)||<\delta$.
From (\ref{eq:xbound}), we have that
\begin{align*}
||\vect{x}||_2^4 \leq \frac{1}{\frac{\epsilon_1(\lambda_{\min}[\tilde{Q}]-K)}{\epsilon_0^2}(t-t_0)+\frac{\epsilon_1}{V(t_0)}} 
\leq \frac{1}{\frac{\epsilon_1}{V(t_0)}} = \frac{V(t_0)}{\epsilon_1} %\leq \frac{\epsilon_0||\vect{x}(t_0)||_2^2}{\epsilon_1} \leq \frac{\epsilon_0\delta^2}{\epsilon_1}
\end{align*}
Since $V(t_0)\leq \epsilon_0||\vect{x}(t_0)||_2^2$,
\begin{align}
||\vect{x}||_2^4\leq \frac{\epsilon_0||\vect{x}(t_0)||_2^2}{\epsilon_1} < \frac{\epsilon_0\delta^2}{\epsilon_1}
\label{eq:bound2}
\end{align}
We would like $||\vect{x}||_2 <\epsilon$ or $||\vect{x}||_2^4 < \epsilon^4$,
%\begin{align*}
%||\vect{x}||_2 &<\epsilon \text{ or }
%||\vect{x}||_2^4 < \epsilon^4
%\end{align*}
so let 
\begin{align*}
\frac{\epsilon_0\delta^2}{\epsilon_1} &<\epsilon^4 \rightarrow
\delta <\epsilon^2\sqrt{\frac{\epsilon_1}{\epsilon_0}}
\end{align*}
